A Directed Cubical Framework for k-critical Bipersistence Modules

In topological data analysis, multiparameter persistence modules (MPMs) are used to analyze data with multiple parameters. Summarizing topological information for MPMs is a non-trivial task; one useful summary of bipersistence modules is the fibered barcode \cite{lesnick2015interactive,lesnick2025fast}. In this paper, we use a directed topological construction of the parameter space of a bifiltration to extend the fibered barcode. Specifically, given a $k$-critical bifiltration $F$, we build an associated directed Euclidean cubical complex $C$ whose directed paths each correspond to a one-parameter subfiltration of $F$. The path space of $C$, $\di{C}$, is used to define the \emph{extended fibered barcode}, which contains all possible monotonically increasing paths in $C$. We show that there can be paths in $\di{C}$ which generate filtrations not obtainable along a line with positive slope, and that all lines with positive slope have a path in $\di{C}$ that generate an equivalent barcode. We introduce two types of equivalence for these restricted modules: combinatorial equivalence of diagrams, and simplicial equivalence of the filtrations generating the modules. We show that removing certain cubes from $C$ yields a subcomplex on which dihomotopic paths induce simplicially equivalent filtrations, and hence combinatorially equivalent diagrams.

==> figs/tixzfigures/bifiltration_K0.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \node[vertexa] at (0.3,.4) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$a$};
\end{scope}

==> figs/tixzfigures/bifiltration_K1.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (0.28,0.35) -- (1.2,0.35);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$a$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$b$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$c$};
\end{scope}

==> figs/tixzfigures/bifiltration_K2.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (0.28,0.35) -- (1.2,0.35);
  \draw[edge] (0.28,0.35) -- (.75,1);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$a$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$b$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$c$};
\end{scope}


==> figs/tixzfigures/bifiltration_K3.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (0.28,0.35) -- (1.2,0.35) -- (.75,1) -- cycle;
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$a$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$b$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$c$};
\end{scope}

==> figs/tixzfigures/bifiltration_K4.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (0.28,0.35) -- (1.2,0.35);
  \draw[edge] (1.2,0.35) -- (.75,1);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$a$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$b$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$c$};
\end{scope}


==> figs/tixzfigures/bifiltration_K5.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  % Fixed canvas: all complex fragments occupy this same square.
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);

  \fill[black!30] (0.28,0.35) -- (1.2,0.35) -- (.75,1) -- cycle;
  \draw[edge] (0.28,0.35) -- (1.2,0.35) -- (.75,1) -- cycle;
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$a$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$b$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$c$};
\end{scope}

==> figs/tixzfigures/bifiltration_K6.tex <==
% Input fragment: use inside a tikzpicture.
% K6 consists of the three isolated vertices [a], [b], and [c].
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$[a]$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$[b]$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$[c]$};
\end{scope}


==> figs/tixzfigures/bifiltration_K7.tex <==
% Input fragment: use inside a tikzpicture.
% K7 consists of [a], [b], [c], and the edge [b,c].
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (1.2,0.35) -- (.75,1);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$[a]$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$[b]$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$[c]$};
\end{scope}


==> figs/tixzfigures/bifiltration_K8.tex <==
% Input fragment: use inside a tikzpicture.
% K8 consists of [a], [b], [c], [a,c], and [b,c].
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (0.28,0.35) -- (.75,1) -- (1.2,0.35);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$[a]$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$[b]$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$[c]$};
\end{scope}


==> figs/tixzfigures/bifiltration_K9.tex <==
% Input fragment: use inside a tikzpicture.
% K7 consists of [a], [b], [c], and the edge [b,c].
\begin{scope}[
  vertexa/.style={circle, fill=violet!85!black, inner sep=2pt},
  vertexb/.style={circle, fill=red!75!black, inner sep=2pt},
  vertexc/.style={circle, fill=green!65!black, inner sep=2pt},
  edge/.style={black, line width=1.35pt, line cap=round}
]
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
  \draw[edge] (0.28,0.35) -- (.75,1);
  \node[vertexa] at (0.28,0.35) {};
  \node[vertexb] at (1.2,0.35) {};
  \node[vertexc] at (.75,1) {};
  \node[anchor=south west, font=\scriptsize] at (0.07,0.07) {$[a]$};
  \node[anchor=south east, font=\scriptsize] at (1.43,0.07) {$[b]$};
  \node[anchor=north, font=\scriptsize] at (.75,1.43) {$[c]$};
\end{scope}


==> figs/tixzfigures/bifiltration_Kempty.tex <==
% Input fragment: use inside a tikzpicture.
\begin{scope}
  \path[use as bounding box] (0,0) rectangle (1.5,1.5);
    \node[anchor=south west] at (0.65,0.65) {$\varnothing$};
\end{scope}
